TaPD: Temporal-adaptive Progressive Distillation for Observation-Adaptive Trajectory Forecasting in Autonomous Driving

Trajectory prediction is essential for autonomous driving, enabling vehicles to anticipate the motion of surrounding agents to support safe planning. However, most existing predictors assume fixed-length histories and suffer substantial performance degradation when observations are variable or extremely short in real-world settings (e.g., due to occlusion or a limited sensing range). We propose TaPD (Temporal-adaptive Progressive Distillation), a unified plug-and-play framework for observation-adaptive trajectory forecasting under variable history lengths. TaPD comprises two cooperative modules: an Observation-Adaptive Forecaster (OAF) for future prediction and a Temporal Backfilling Module (TBM) for explicit reconstruction of the past. OAF is built on progressive knowledge distillation (PKD), which transfers motion pattern knowledge from long-horizon "teachers" to short-horizon "students" via hierarchical feature regression, enabling short observations to recover richer motion context. We further introduce a cosine-annealed distillation weighting scheme to balance forecasting supervision and feature alignment, improving optimization stability and cross-length consistency. For extremely short histories where implicit alignment is insufficient, TBM backfills missing historical segments conditioned on scene evolution, producing context-rich trajectories that strengthen PKD and thereby improve OAF. We employ a decoupled pretrain-reconstruct-finetune protocol to preserve real-motion priors while adapting to backfilled inputs. Extensive experiments on Argoverse 1 and Argoverse 2 show that TaPD consistently outperforms strong baselines across all observation lengths, delivers especially large gains under very short inputs, and improves other predictors (e.g., HiVT) in a plug-and-play manner. Code will be available at https://github.com/zhouhao94/TaPD.

==> table/table_av1_compare.tex <==
\begin{table}[t!]
% \begin{}
\caption{Performance with Different Timesteps on {\it Argoverse 1 single-agent validation set}.}
\label{tab:av1_compare}
\centering
\begin{tabular}{l cccc}
\toprule[1.5pt]
\multirow{2}{*}{Method} & 
\multicolumn{4}{c}{$\textit{minADE}_{6}$ / $\textit{minFDE}_{6}$} \\
\cmidrule(lr){2-5}    % 添加行线
% & 10Ts & 20Ts & 30Ts & 40Ts & 50Ts 
& 5Ts & 10Ts & 15Ts & 20Ts \\
[1.5pt]\hline\noalign{\vskip 2pt}
DeMo\_Ori
% &9.999/9.999& 9.999/9.999 &1.649/4.119 &1.623/4.067 &1.608/4.033     % ADE1/FDE1
& 0.781/1.267  &0.662/1.087 &0.624/1.011 &0.606/1.003 \\    % ADE6/FDE6
DeMo\_IT 
% & 9.999/9.999 & 9.999/9.999 & 1.606/4.038 & 1.605/4.062 & 1.608/4.033 
& 0.669/1.078 & 0.634/1.031 &0.612/0.988 & 0.606/1.003  \\
DeMo\_DTO
& 0.662/1.064 & 0.628/1.025 &0.605/0.991 &0.599/1.010 \\
DeMo\_FLN
& 0.646/1.043 & 0.607/0.994 & 0.599/0.974 & 0.592/0.957 \\
DeMo\_LaKD
& \underline{0.631}/1.008 & 0.593/0.976 & 0.584/0.933 & 0.581/0.929 \\
DeMo\_CLLS
& 0.634/\underline{0.998} & \underline{0.587}/\underline{0.959} & \underline{0.580}/\underline{0.919} & \underline{0.579}/\underline{0.922} \\
DeMo\_TaPD(Ours)
& \bf 0.608/\bf 0.974 & \bf 0.574/\bf 0.915 & \bf 0.573/\bf 0.914 & \bf 0.573/\bf 0.914\\
[1.5pt]\hline\noalign{\vskip 2pt}
\end{tabular}
\end{table}

==> table/table_av2_single_test.tex <==
\begin{table*} [ht!]
    \caption{Performance comparison on {\it Argoverse 2 single-agent test set} in the official leaderboard. For each metric, the best result is in \textbf{bold} and the second best result is \underline{underlined}.}
    \label{tab:av2_single}
    \centering
    % \vspace{1em}
    {\begin{tabular}{l|cccccc}
       \toprule[1.5pt]
        $\textbf{Method}$ & $\textit{minFDE}_{1}$ & $\textit{minADE}_{1}$ & $\textit{minFDE}_{6}$ & $\textit{minADE}_{6}$ & $\textit{MR}_{6}$ & $\textit{b-minFDE}_{6}$\textit{}\\
        [1.5pt]\hline\noalign{\vskip 2pt}
        FRM~\cite{frm}              & 5.93 & 2.37 & 1.81 & 0.89 & 0.29 & 2.47\\
        HDGT~\cite{hdgt}            & 5.37 & 2.08 & 1.60 & 0.84 & 0.21 & 2.24\\  
        SIMPL~\cite{simpl}          & 5.50 & 2.03 & 1.43 & 0.72 & 0.19 & 2.05\\
        THOMAS~\cite{thomas}        & 4.71 & 1.95 & 1.51 & 0.88 & 0.20 & 2.16\\
        GoRela~\cite{gorela}        & 4.62 & 1.82 & 1.48 & 0.76 & 0.22 & 2.01\\ 
        MTR\cite{mtr}               & 4.39 & 1.74 & 1.44 & 0.73 & 0.15 & 1.98\\
        HPTR~\cite{HPTR}            & 4.61 & 1.84 & 1.43 & 0.73 & 0.19 & 2.03\\
        GANet~\cite{ganet}          & 4.48 & 1.77 & 1.34 & 0.72 & 0.17 & 1.96\\
        ProphNet~\cite{prophnet}    & 4.74 & 1.80 & 1.33 & 0.68 & 0.18 & 1.88 \\  
        QCNet~\cite{qcnet}          & 4.30 & 1.69 & 1.29 & 0.65 & 0.16 & 1.91\\   
        SmartRefine~\cite{smartrefine}     & 4.17 & 1.65 & \underline{1.23} & \underline{0.63} & \underline{0.15} & \underline{1.86}\\
        DeMo~\cite{demo}            & \underline{4.09} & \underline{1.63} & 1.28 & 0.67 & 0.16 & 1.95 \\     
        \hline\noalign{\vskip 2pt}
        \bf\netName~(Ours)  & \bf 3.91 &  \bf 1.53 & \bf 1.17 & \bf 0.61 &\bf 0.13 & \bf 1.85 \\
        [1.5pt] \hline\noalign{\vskip 2pt}

    \end{tabular}}
\end{table*}


